Circum- and Inconic Invariants of 3-Periodics in the Elliptic Billiard

A Circumconic passes through a triangle's vertices; an Inconic is tangent to the sidelines. We study the variable geometry of certain conics derived from the 1d family of 3-periodics in the Elliptic Billiard. Some display intriguing invariances such as aspect ratio and pairwise ratio of focal lengths.

==> _not_used/020_circumbilliard.tex <==
Let the boundary of the EB satisfy:

\begin{equation}
\label{eqn:billiard-f}
f(x,y)=\left(\frac{x}{a}\right)^2+\left(\frac{y}{b}\right)^2=1.
\end{equation}

Where $a>b>0$ denote the EB semi-axes throughout the paper. Below we use {\em aspect ratio} as the ratio of an ellipse's semi-axes. When referring to Triangle Centers we adopt Kimberling $X_i$ notation \cite{etc}, e.g., $X_1$ for the Incenter, $X_2$ for the Barycenter, etc., see Table~\ref{tab:kimberling} in Appendix~\ref{app:symbols}.

The following five-parameter equation is assumed for all circumconics not passing through $(0,0)$.

\begin{equation}
1 + c_1 x + c_2 y + c_3 x y + c_4 x^2 + c_5 y^2=0
\label{eqn:e0}
\end{equation}

\begin{proposition}
Any triangle $T=(P_1,P_2,P_3)$ is associated with a unique 
ellipse $E_9$ for which $T$ is a billiard 3-periodic. The center of $E_9$ is T's Mittenpunkt.
\end{proposition}

\begin{proof}
If $T$ is a 3-periodic of $E_9$, by Poncelet's Porism, $T$ is but an element of a 1d family of 3-periodics, all sharing the same confocal Caustic\footnote{This turns out to be the Mandart Inellipse $I_9$ of the family \cite{mw}.}. This family will share a common Mittenpunkt $X_9$ located at the center of $E_9$  \cite{reznik2020-intelligencer}. Appendix~\ref{app:circum-linear} shows how to obtain the parameters for \eqref{eqn:e0} such that it passes through $P_1,P_2,P_3$ and is centered on $X_9$: this yields a $5{\times}5$ linear system. Solving it its is obtained a quadratic equation with positive discriminant, hence the conic is an ellipse.
\end{proof}

$E_9$ is called the Circumbilliard (CB) of $T$. Figure~\ref{fig:circumbilliard} shows examples of CBs for two sample triangles.

\begin{figure}[H]
    \centering
    \includegraphics[width=.8\textwidth]{pics_eps_new/0010_circumplot}
    \caption{Two random triangles are shown as well as their Circumbilliards (CBs). Notice their axes in general are not horizontal/vertical. An algorithm for computing the CB is given in Appendix~\ref{app:circum-linear}. \textbf{Video:} \cite[PL\#02]{reznik2020-playlist-circum}}
    \label{fig:circumbilliard}
\end{figure}




==> _not_used/030_cb_derived.tex <==
Figure~\ref{fig:cb_trio} shows CBs for the Excentral, Anticomplementary (ACT), and Medial Triangles, derived from 3-periodics.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics_eps_new/0020_cb_trio.eps}
    \caption{Draw in black in each picture is an $a/b=\varphi{\simeq}1.618$ EB and a 3-periodic at $t=7.0^\circ$. \textbf{Left}: the CB of the Excentral Triangle (solid green) centered on the latter's Mittenpunkt is $X_{168}$ \cite{etc}. Its locus (red) is non-elliptic. Also shown (dashed green) is the elliptic locus of the Excenters (the MacBeath Circumellipse $E_6'$ of the Excentrals \cite{mw}), whose center is $X_9$ \cite{garcia2020-ellipses}; \textbf{Top Right}: the CB of the Anticomplementary Triangle (ACT) (blue), axis-aligned with the EB. Its center is the Gergonne Point $X_7$, whose locus (red) is elliptic and similar to the EB \cite{garcia2020-ellipses}. The locus of the ACT vertices is not elliptic (dashed blue); \textbf{Bottom Right}: the CB of the Medial Triangle (teal), also axis-aligned with the EB, is centered on $X_{142}$, whose locus (red) is also elliptic and similar to the EB, since it is the midpoint of $X_9X_7$ \cite{etc}. The locus of the medial vertices is a dumb-bell shaped curve (dashed teal). \textbf{Video:} \cite[PL\#03]{reznik2020-playlist-circum}}
    \label{fig:cb_trio}
\end{figure}


\subsection{Excentral Triangle}
\label{sec:cb_exc}

The locus of the Excenters is shown in Figure~\ref{fig:cb_trio} (left). It is an ellipse similar to the $90^\circ$-rotated locus of $X_1$ and its axes $a_e,b_e$ are given by \cite{garcia2019-incenter,garcia2020-ellipses}:

\begin{equation*}
 a_e=\frac{{b}^{2}+\delta}{a},\;\;\; 
 b_e=\frac{{a}^{2}+\delta}{b}
\end{equation*}

Where $\delta=\sqrt{a^4-a^2 b^2+b^4}$. 

\begin{proposition}
The locus of the Excenters the stationary MacBeath Circumellipse $E_6'$ \cite{mw} of the Excentral Triangles.
\end{proposition}

\begin{proof}
The center of $E_6'$ is the Symmedian Point $X_6$ \cite[MacBeath Circumconic]{mw}. The Excentral Triangle's $X_6$ coincides with the Mittenpunkt $X_9$ of the reference \cite{etc}. Since over the 3-periodics the vertices of the Excentral lie on an ellipse and its center is stationary, the result follows.
\end{proof}

\begin{proposition}
The Excentral CB is centered on $X_{168}$, whose trilinears are irrational, and whose locus is non-elliptic.
\end{proposition}

\begin{proof}
$X_{168}$ is the Mittenpunkt of the Excentral Triangle \cite{etc} and its trilinears are irrational\footnote{No Triangle Center whose trilinears are irrational on sidelengths has yet been found whose locus under the 3-periodic family is an ellipse \cite{garcia2020-ellipses}.} on the sidelengths. To determine if its locus is an ellipse we use the algebro-numeric techniques described in \cite{garcia2020-ellipses}. Namely, a least-squares fit of a zero-centered, axis-aligned ellipse to a sample of $X_{168}$ positions of the 3-periodic family produces finite error, therefore it cannot be an ellipse.
\end{proof}

This had been observed in \cite{garcia2020-ellipses} for several irrational centers such as $X_i,i=$13--18, as well as many others. Notice a center may be rational but produce a non-elliptic locus, the emblematic case being $X_6$, whose locus is a convex quartic. Other examples include $X_j,j=$19, 22--27, etc.

\subsection{Anticomplementary Triangle (ACT)}
\label{sec:cb_act}

The ACT is shown in Figure~\ref{fig:cb_trio} (top right). The locus of its vertices is clearly not an ellipse.

The ACT is perspective with the reference triangle (3-periodic) at $X_2$ and all of its triangle centers correspond to the anticomplement\footnote{Anticomplement: a 1:2 reflection about $X_2$.} of corresponding reference ones \cite{mw}. The center of the CB of the ACT is therefore $X_7$, the anticomplement of $X_9$. We have shown the locus of $X_7$ to be an ellipse similar to the EB with axes \cite{garcia2020-ellipses}:

\begin{equation*}
\left(a_7,b_7\right)=k\left(a,b\right),\;\;\text{with: }k=\frac{2\delta - {a}^{2}-{b}^{2}}{a^2-b^2}
\end{equation*}

\begin{remark}
The axes of the ACT CB are parallel to the EB and of fixed length.
\end{remark}

This stems from the fact the ACT is homothetic to the 3-periodic.

\subsection{Medial Triangle}

The locus of its vertices is the dumbbell-shaped curve, which at larger $a/b$ is self-intersecting, and therefore clearly not an ellipse, Figure~\ref{fig:cb_trio} (bottom right).

Like the ACT, the Medial is perspective with the reference triangle (3-periodic) at $X_2$. All of its triangle centers correspond to the complement\footnote{Complement: a 2:1 reflection about $X_2$.} of corresponding reference ones \cite{mw}. The center of the CB of the Medial is therefore $X_{142}$, the complement of $X_9$. This point is known to sit midway between $X_9$ and $X_7$.

\begin{remark}
The locus of $X_{142}$ is an ellipse similar to the EB.
\end{remark}

This stems from the fact $X_9$ is stationary and the locus of $X_7$ is an ellipse similar to the EB (above). Therefore its axes will be given by:

\begin{equation*}
\left(a_{142},b_{142}\right)=(a_7,b_7)/2
\end{equation*}

Stemming from homothety of 3-periodic and its Medial:

\begin{remark}
The axes of the Medial CB are parallel to the EB and of fixed length.
\end{remark}

\subsection{Superposition of ACT and Medial}

\begin{proposition}
The Intouchpoints of the ACT (resp. 3-periodic) are on the EB (resp. on the CB of the Medial)
\end{proposition}

\begin{proof}
The first part was proved in \cite[Thm. 2]{reznik2020-ballet}. Because the 3-periodic can be regarded as the ACT of the Medial, the result follows.
\end{proof}

This phenomenon is shown in Figure~\ref{fig:cb_act_med_superposed}. Also shown is the fact that $X_i,i=$7, 142, 2, 9, 144 are all collinear and their intermediate intervals are related as $3:1:2:6$. In \cite{etc_central_lines} this line is known as $L(X_2,X_7)$ or $\mathcal{L}_{663}$. $X_{144}$ is the perspector of the ACT and its Intouch Triangle (not shown).
%\begin{align*}
%a(b - c)(b + c - a)x &+ \\
%b(c - a)(c + a - b)y &+ \\
%c(a - b)(a + b - c)z &= 0
%\end{align*}
%I.e., it is L(663), since
%$$X(663) = a(b - c)(b + c - a) ::$$
%Passes through: 2 7 9 57 63 142 144 226 307 329 527 553 579 672 894 908 1025 1400 1423 1445 1447 1652 1653 1708 1741 1944 2002 2094 2285 2406


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics_eps_new/0120_actMedCircumAll.eps}
    \caption{Construction for both ACT and Medial CBs, centered on $X_7$ and $X_{142}$, respectively. The Incircle of the ACT (resp. 3-periodic) is shown blue (resp. green). The former touches the ACT at the EB and the latter touches the 3-periodic sides at the Medial CB. Also shown is line $L(2,7)=L_{663}$ which cointains $X_i$, $i=7,142,2,9,144$. Their consecutive distances are proportional to $3:1:2:6$. $X_{144}$ was included since it is the perspector of the ACT and its Intouch Triangle (not shown) \cite{mw}. \textbf{Video}: \cite[PL\#04,05]{reznik2020-playlist-circum}}
    \label{fig:cb_act_med_superposed}
\end{figure}

\input{035_cb_orthic}

\subsection{Summary}

Table~\ref{tab:cb_summary} summarizes the CBs discussed above, their centers, and their loci.

\begin{table}[H]
\begin{tabular}{|c|c|c|}
\hline
Triangle & Center & Elliptic Locus \\
\hline
3-Periodic & $X_9$ & n/a \\
Excentral & $X_{168}$ & No\\
ACT & $X_{7}$ & Yes \\
Medial & $X_{142}$ & Yes \\
Orthic & $X_6^*$ & No \\
\hline
\end{tabular}
\caption{CBs mentioned in this Section, their Centers and loci types.}
\label{tab:cb_summary}
\end{table}

\subsection{Circumbilliard of the Poristic Family}

The Poristic Triangle Family is a set of triangles (blue) with fixed Incircle and Circumcircle \cite{gallatly1914-geometry}. It is a cousing of the 3-periodic family in that by definition its Inradius-to-Circumradius $r/R$ ratio is constant.

Weaver \cite{weaver1927-poristic} proved the Antiorthic Axis\footnote{The line passing through the intersections of reference and Excentral sidelines \cite{mw}.} of this family is stationary. Odehnal showed the locus of the Excenters is a circle centered on $X_{40}$ and of radius $2R$ \cite{odehnal2011-poristic}. He also showed that over the family, the locus of the Mittenpunkt $X_9$ is a circle whose radius is $2{d^2}(4R+r)$ and center is $X_1 + (X_1 - X_3) (2 R - r)/(4 R + r)$, where $d=|X_1X_3|=\sqrt{R(R-2{r})}$ \cite[page 17]{odehnal2011-poristic}.

Let $\rho=r/R$ and $a_9,b_9$ be the semi-axis lengths of the Circumbilliard a poristic triangle. As shown in Figure~\ref{fig:cb-poristic}:

\begin{theorem}
The ratio $a_9/b_9$ is invariant over the family and is given by:

\begin{equation*}
\frac{a_9}{b_9}=\sqrt{\frac{\rho^2+2 (\rho+1)\sqrt{1-2\rho} +2}{\rho (\rho+4)}}
\end{equation*}
\noindent where $\rho=r/R$.
\label{thm:poristic}
\end{theorem}

\begin{proof}
The following expression for $r/R$ has been derived for the 3-periodic family of an $a,b$ EB \cite[Equation 7]{garcia2020-new-properties}:

\begin{equation}
  \rho = \frac{r}{R} =  \frac{2(\delta-b^2)(a^2-\delta)}{ (a^2-b^2)^2}
\end{equation}
Solving the above for $a/b$ yields the result.
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics_eps_new/0160_poristic_cb.eps}
    \caption{Two configurations (left and right) of the Poristic Triangle Family (blue), whose Incircle (green) and Circumcircle (purple) are fixed. Here $R=1,r=0.3625$. Over the family, the Circumbilliard (black) has invariant aspect ratio, in this case $a_9/b_9{\simeq}1.5$. Also shown is the circular locus of $X_9$ \cite[page 17]{odehnal2011-poristic}. \textbf{Video}: \cite[PL\#07]{reznik2020-playlist-circum}.}
    \label{fig:cb-poristic}
\end{figure}

==> _not_used/035_cb_orthic.tex <==
\subsection{Orthic Triangle}
\label{sec:cb_ort}

Let $\alpha_4=\sqrt{2\,\sqrt {2}-1}\;{\simeq}\;1.352$. In \cite[Thm. 1]{reznik2020-ballet} we show that if $a/b>\alpha_4$, the 3-periodic family will contain obtuse triangles.

\begin{proposition}
If $a/b>\alpha_4$, the 3-periodic is a right triangle when one of its vertices is at four symmetric points $P^\perp_i$, $i=1,2,3,4$ given by $({\pm}x^\perp,{\pm}y^\perp)$ with:

\begin{equation}
x^\perp=\frac{a^2 \sqrt{a^4+3 b^4-4 b^2 \delta }}{c^3},\;\;\;
y^\perp=\frac{b^2 \sqrt{-b^4-3 a^4+4 a^2 \delta }}{c^3}
\label{eqn:perp}
\end{equation}
\label{prop:right-triangle}
\end{proposition}

\begin{proof}
Let the coordinates of the 3-periodic vertices be $P_1=(x_1,y_1),P_2=(x_2,y_2),P_3=(x_3,y_3)$   as derived in \cite{garcia2019-incenter}.

Computing the equation $\langle P_2-P_1,P_3-P_1\rangle=0$, after careful algebraic manipulations, it follows that $x_1$ satisfies the quartic equation
\[ c^8 x_1^4-2a^4c^2(a^4+3b^4)x_1^2+a^8(a^4+2a^2b^2-7b^4)=0.\] 
For $a/b>\sqrt{2\sqrt{2}-1} $ the only
  positive root in the interval $(0,a)$ is given by

\begin{equation}
x^{\perp}=\frac{a^2 \sqrt{a^4+3 b^4-4 b^2 \delta }}{c^3}.
\label{eqn:xperp}
\end{equation}

\noindent With $y^\perp$ obtainable from \eqref{eqn:billiard-f}.
\end{proof}

Equivalently, a 3-periodic will be obtuse iff one of its vertices lies on top or bottom halves of the EB between the $P_i^\perp$, see Figure~\ref{fig:rect_zones}.

\begin{figure}
    \centering
    \includegraphics[width=.66\textwidth]{pics_eps_new/0080_rect_zones.eps}
    \caption{Two 3-periodics are shown: one acute (solid blue) and one obtuse (dashed blue) inscribed into an $a/b=1.618$ EB. Red arcs along the top and bottom halves of the EB indicate that when a 3-periodic vertex is there, the 3-periodic is obtuse. These only exist when $a/b>\alpha_4{\simeq}1.352$.}
    \label{fig:rect_zones}
\end{figure}

Consider the elliptic arc along the EB between $({\pm}x^\perp,y^\perp)$. When a vertex of the 3-periodic lies within  (resp. outside) this interval, the 3-periodic is obtuse (resp. acute).

\begin{proposition}
When $a/b>\alpha_4$, the locus of the center of the Orthic CB has four pieces: 2 for when the 3-periodic is acute (equal to the $X_6$ locus), and 2 when it is obtuse (equal to the locus of $X_6$ of $T''=P_2P_3X_4$.
\end{proposition}

\begin{proof}
It is well-known that \cite{etc} an acute triangle $T$ has an Orthic whose vertices lie on the sidelines. Furthermore the Orthic's Mittenpunkt coincides with the Symmedian $X_6$ of $T$. Also known is the fact that:

\begin{remark}
Let triangle $T'=P_1P_2P_3$ be obtuse on $P_1$. Its Orthic has one vertex on $P_2P_3$ and  two others exterior to $T'$. Its Orthocenter $X_4$ is also exterior. Furthermore, the Orthic's Mittenpunkt is the Symmedian Point $X_6$ of acute triangle $T''=P_2P_3X_4$.
\end{remark}

To see this, notice the Orthic of $T''$ is also\footnote{The anti-orthic pre-images of $T'$ are both the 3-periodic and $T''$.} $T'$. $T''$ must be acute since its Orthocenter is $P_2$.
\end{proof}

The CB of the orthic is shown in Figures~\ref{fig:cb_ort} for four 3-periodic configurations in an EB whose $a/b>\alpha_4$.

\begin{proposition}

The coordinates $({\pm}x^*,{\pm}y^*)$ where the locus of the center of the Orthic's CB transitions from one curve to the other are given by:

\begin{align*}
x^*=&\frac{x^{\perp}}{c^6}\left(a^6+2 a^2 b^4- b^2 \delta(3 a^2  +b^2)    +b^6\right)\\
%\frac{a^2 \sqrt{a^4+3 b^4-4 b^2 \delta } \left(a^6+2 a^2 b^4-3 a^2 b^2 \delta +b^6-b^4 \delta \right)}{c^9} \\
%=\frac{a^2 x^{\perp}}{a^2+b^2} \\
y^* =&-\frac{y^{\perp}}{c^6}\left(b^6+2 a^4 b^2 -  a^2 \delta (3 b^2 +a^2)   \delta+a^6\right)
   %\frac{b^2 \sqrt{-3 a^4+4
 %  a^2 \delta -b^4} \left(-a^6-2 a^4 b^2+a^4 \delta +3 a^2 b^2 \delta -b^6\right)}{c^9}\\
  % =\frac{b^2y^{\perp}}{a^2+b^2}
\end{align*}

\end{proposition}

\begin{proof}
Let $P_1=(x_1,y_1)$ be the right-triangle vertex of a 3-periodic, given by $(x^\perp,y^\perp)$ as in \eqref{eqn:xperp}. Using \cite{garcia2019-incenter}, obtain $P_2=(p_{2x}/q_2, p_{2y}/q_2)$ and $P_3=(p_{3x}/q_3, p_{3y}/q_3)$, with:
 
 \begin{align*}
     p_{2x}= &b^4 c^2 x_1^3 -2 a^4 b^2 x_1^2 y_1+a^4 c^2 x_1 y_1^2-2 a^6 y_1^3\\
     %
     p_{2y}=&2 b^6 x_1^3-b^4 c^2  x_1^2 y_1+2 a^2 b^4x_1 y_1^2-a^4 c^2 y_1^3\\
     q_2=&b^4 (a^2+b^2) x_1^2-2 a^2 b^2c^2 x_1 y_1 +a^4 (a^2+b^2) y_1^2\\
     p_{3x}=& b^4 c^2 x_1^3  +2 a^4 b^2 x_1^2 y_1+a^4 c^2 x_1 y_1^2+a^6 y_1^3\\
     p_{3y}=&-2 b^6 x_1^3 -b^4 c^2 x_1^2 y_1-2 a^2 b^4 x_1 y_1^2-a^4 c^2 y_1^3 \\
     q_3=&b^4 (a^2+b^2) x_1^2+2 a^2 b^2c^2 x_1 y_1+a^4 (a^2+b^2) y_1^2
 \end{align*}


It can be shown the Symmedian point $X_6$ of a right-triangle is the midpoint of its right-angle vertex altitude. Computing $X_6$ using this property leads to the result.
\end{proof}

    
Let $\alpha_{eq}=\sqrt{4 \sqrt{3}-3}\,{\simeq}\,1.982$ be the only positive root of $x^4 + 6 x^2 - 39$. It can be shown, see Figure~\ref{fig:cb_ort_equi}:

\begin{proposition}
At $a/b=\alpha_{eq}$, the locus of the Orthic CB is tangent to EB's top and bottom vertices. If a 3-periodic vertex is there, the Orthic is equilateral.
\end{proposition}

\begin{proof}
Let $T$ be an equilateral with side $s_{eq}$ and center $C$. Let $h$ be the distance from any vertex of $T$ to $C$. It can be easily shown that $h/s_{eq}=\sqrt{3}/3$. Let $T'$ be the Excentral Triangle of $T$: its sides are $2s_{eq}$. Now consider the upside down equilateral in Figure~\ref{fig:cb_ort_equi}, which is the Orthic of an upright isosceles 3-periodic. $h$ is clearly the 3-periodic's height and $2s_{eq}$ is its base. The height and width of the upright isosceles are obtained from explicit expressions for the vertices \cite{garcia2019-incenter}:

\begin{align*}
    s_{eq}=\frac{\alpha^2}{\alpha^2-1}\sqrt{2\delta-\alpha^2-1},\;\;\;h=\frac{\alpha^2+\delta+1}{\alpha^2+\delta}
\end{align*}

\noindent where $\alpha=a/b$. Setting $h/s_{eq}=\sqrt{3}/3$ and solving for $\alpha$ yields the required result for $\alpha_{eq}$.
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics_eps_new/0030_cb_ort.eps}
    \caption{Orthic CB for an EB with $a/b=1.5>\alpha_4$, i.e., containing obtuse 3-periodics, which occur when a 3-periodic vertex lies on the top or bottom areas of the EB between the $P^\perp$. \textbf{Top left}: 3-periodic is sideways isosceles and acute (vertices outside $P^\perp$, so 3 orthic vertices lie on sidelines. The Orthic CB centers is simply the mittenpunkt of the Orthic, i.e, $X_6$ of the 3-periodic (blue curve: a convex quartic \cite{garcia2020-ellipses}). \textbf{Top right}: The position when a vertex is at a $P^\perp$ and the 3-periodic is a right triangle: its Orthic and CB degenerate to a segment. Here the CB center is at a first (of four) transition points shown in the other insets as $Q_i$, $i=1,2,3,4$. \textbf{Bottom left}: The 3-periodic is obtuse, the Orthic has two exterior vertices, and the center of the CB switches to the Symmedian of $T''=P_1P_2X_4$ (red portion of locus). \textbf{Bottom right:}. The 3-periodic is an upright isosceles, still obtuse, the center of the Orthic CB reaches its highest point along its locus (red). \textbf{Video}: \cite[PL\#06]{reznik2020-playlist-circum}.}
    \label{fig:cb_ort}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics_eps_new/0040_cb_ort_equi.eps}
    \caption{At $a/b=\alpha_{eq}{\simeq}1.982$, the Orthic is an equilateral triangle when a 3-periodic vertex lies on a top or bottom vertex of the EB. Therefore its CB is a circle.}
    \label{fig:cb_ort_equi}
\end{figure}

==> _not_used/099_pythagorean.tex <==
We have seen \cite{ronaldo2020-loci} that with $a/b>a_4=\sqrt{2\,\sqrt{2}-1}\simeq{1.352}$ the orbit family contains obtuse triangles amongst which there always are 4 right triangles (identical up to rotation and reflection). An interesting question is which EB aspect ratios produce primitive {\em Pythagorean} triangles, i.e., right triangles with sides $s_1,s_2,s_3$ for which $s_1,s_2$ are co-prime, and $s_3^2=s_1^2+s_2^2$.

Start with an elementary Pythagorean triangle $P_1=(0,0)$, $P_2=(s_1,0)$, and $P_3=(s_1,s_2)$ choosing $s_1,s_2$ integers such that $s_3=s_3=\sqrt{s_1^2+s_2^2}$ is an integer.
The Circumbilliard is given by
\[
E_9(x,y)= s_2 x^2+ \left( s_3-s_1-s_2 \right) xy+s_1{y}^{2}-s_1s_2x-s_1 \left( s_1-s_3 \right) y=0.\]

Computing the axes of its Circumbilliard we obtain: 

\begin{equation}
    [a/b](s_1,s_2,s_3)= \frac {s_1+s_2+\sqrt {s_3\left(3\,s_3-2\,s_1-2\,s_2\right) }}{\sqrt { \left( 
s_1+s_2+3\,s_3 \right)  \left( s_1+s_2-s_3 \right) }}
\end{equation}

%\begin{equation*}
  %  \lim_{s_2\to \infty} %r(s_2,s_2,\sqrt{2}s_2)=\sqrt{2\sqrt{2}-1}\simeq %1.352
%\end{equation*}
%The axis of the Circumbilliard are:

%\begin{align}
%    a(m,n,p)=&  \\
 %   b(m,n,p)=&
%\end{align}

Table~\ref{tab:pythagorean} shows the aspect ratios required for the first 16 Pythagorean triples ordered by hypotenuse\footnote{The $a/b$ which produces $3:4:5$ was first computed in \cite{ronaldo2020-loci} in connection with $X_{88}$.}

\begin{table}[H]
\scriptsize
$$
\begin{array}{r|c|l|l}
(s_1,s_2,s_3) & a/b & {\simeq}a/b & \text{isosc. rank} \\
\hline
3, 4, 5 & {(7+\sqrt{5})\sqrt{11}}/{22} &  1.392 &  4 \\
5, 12, 13 & {\sqrt{14} (\sqrt{65}+17)}/{56} & 1.674 &  10 \\
8, 15, 17 & {\sqrt{111} (\sqrt{85}+23)}/{222} & 1.529 & 8\\
7, 24, 25  & {\sqrt{159} (5\,\sqrt{13}+31)}/{318} & 1.944 & 12 \\
\mathbf{20, 21, 29} & \mathbf{\sqrt{6} (\sqrt{145}+41)/{96}} & \mathbf{1.353} &  \mathbf{1} \\
12, 35, 37 & {\sqrt{395} (\sqrt{629}+47)}/{790} & 1.813 & 11 \\
9, 40, 41 & {\sqrt{86} (5\,\sqrt{41}+49)}/{344}& 2.184 &  14 \\
28, 45, 53 & {\sqrt{290} (\sqrt{689}+73)}/{1160} & 1.457 & 5 \\
11, 60, 61 & {\sqrt{635} (\sqrt{2501}+71)}/{1270} & 2.401 & 15 \\
16, 63, 65 & {\sqrt{959} (\sqrt{2405}+79)}/{1918} & 2.067 & 13 \\
33, 56, 65 & {\sqrt{426} (\sqrt{1105}+89)}/{1704} & 1.481  & 6 \\
48, 55, 73 & {\sqrt{2415} (\sqrt{949}+103)}/{4830} & 1.361 &  3 \\
\mathbf{13, 84, 85} & \mathbf{\sqrt{66} (97+\sqrt{5185})/{528}} & \mathbf{2.600} & \mathbf{16} \\
36, 77, 85 & {\sqrt{161} (\sqrt{2465}+113)}/{1288} & 1.602 & 9 \\
39, 80, 89 & {\sqrt{2895} (\sqrt{2581}+119)}/{5790} & 1.578 &  8 \\
65, 72, 97 & {\sqrt{1070} (\sqrt{1649}+137)}/{4280}& 1.357 & 2
\end{array}
$$
%\[a/b_{\perp}(m,n,p)=\sqrt {{\frac {m+n+\sqrt {p %( -2\,m-2\,n+3\,p \right) }}{m+n-
%\sqrt {p ( -2\,m-2\,n+3\,p \right) }}}}\]
\caption{The first column shows the first 16 Pythagorean triples ordered by hypotenuse $s_3$. The second one shows the $a/b$ family which produces it. The boldfaced triple $(20,21,29)$ (resp.~$(13,84,85)$) is the closest (resp.~farthest) to an isosceles in the table. This means $a/b$ will be closest to $a_4=1.352$. If rows were listed in ascending order of  $|s_1/s_2-1|$ (how scalene a triple is), the values of $a/b$ would also appear ascending, as indicated by the ``rank'' column.}
\label{tab:pythagorean}
\end{table}
%


\subsection{First 12k Pythagoreans in $a,b$ space}

Euclid's Algorithm generates a primitive Pythagorean triple from a co-prime pair $m,n$, $m>n$. For example, $(3,4,5)$ (resp.~$(5,12,13)$) is generated with $m=2,n=1$ (resp., $m=3,n=2$), etc.

Figure~\ref{fig:pythagorean} shows the first 12231 triangles generated in this fashion with $1<m<200$ in both $(s_1,s_2)$ and $(a,b)$ space. A few interesting observations are given in the caption. 

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{pics_eps/0101_pythagorean_legs_ab.eps}
    \caption{\textbf{Top}: Right-triangles generated by Euclid's Algorithm with $n<m<200$, $m,n$ co-prime. Roughly 12k $(s_1,s_2)$ leg combinations are shown as black dots. To save space, the y-axis is drawn half-scale and points with $s_2>50000$ are not drawn. The green line represents $s_1=s_2$, i.e., isosceles triangles (only quasi-isosceles can be generated). The red (resp.~blue) curve is drawn over triangles obtained with $m=150$ (resp.~$n=150$). \textbf{Bottom}: Axes $(a,b)$ combinations which can produce the aforementioned right-triangles. The point cloud is properly under the green line $a/b=a_4$ (aspect ratio which produces an isosceles right-triangle). The constant $m=150$ (resp.~$n=150$) runs produce a red (resp.~blue) arch in $(a,b)$ space. Quasi-similar triangles organize in straight lines from the origin toward the right, i.e., they are generated by quasi-similar billiards.}
    \label{fig:pythagorean}
\end{figure}

\subsection{Iso-perimetric Primitive Pythagoreans}

Out of the 12231 Pythagorean triples generated, only 11548 perimeters $s_1+s_2+s_3$ are unique. Out of these, 10912 are associated with a single triple. An additional 585 (resp.~47) unique perimeters are each produced by two (resp.~3) distinct triples. Finally, 2 unique perimeters -- 60060 and 78540 -- are shared by two distinct groups of four triples, listed below:

$$
\scriptsize
\begin{array}{|c|c|c|c|}
\hline
\text{L} & s_1 & s_2 & s_3 \\
\hline
 60060 & 6699 & 26260 & 27101 \\
 60060 & 15960 & 19162 & 24938 \\
 60060 & 22035 & 12628 & 25397 \\
 60060 & 26936 & 5610 & 27514 \\
 78540 & 13515 & 31108 & 33917 \\
 78540 & 21896 & 24090 & 32554 \\
 78540 & 25179 & 20740 & 32621 \\
 78540 & 34440 & 8602 & 35498 \\
 \hline
\end{array}
$$

The perimeter $L$ of a 3-periodic orbit as a function of the EB axes $a,b$ is given by \cite{ronaldo2020-loci}:

\begin{equation*}
L=\frac{2(\delta+a^2+b^2)\sqrt{2\delta-a^2-b^2}}{a^2-b^2}
\end{equation*}

\noindent with $\delta=\sqrt(a^4-a^2 b^2+b^4)$. Each $L$ defines a level curve in $(a,b)$ space\footnote{Given by the quartic $(a^2-b^2)^2 L^4-(2(2a^2-b^2))(a^2-2 b^2)(a^2+b^2) L^2-27 a^4 b^4=0$.} which represents a 1d family of EBs such that all their orbit families have the same perimeter, see Figure~\ref{fig:iso-perimeter-3-and-4}.

The two groups of 4 triples with the same perimeter are shown in Figure~\ref{fig:iso-perimeter-4} against level curves of their perimeter. A similar picture for the 4-groups and 3-groups is shown in Figure~\ref{fig:iso-perimeter-3-and-4}.

\begin{figure}[H]
    \centering
    \includegraphics[width=.66\textwidth]{pics_eps/0120_fourTriplesPlot.eps}
    \caption{Two iso-perimetric curves are shown in $(a,b)$ space corresponding to EB families whose orbits have the same perimeter. Also shown are the 4-member groups of primitive Pythagorean triples sharing either perimeter.}
    \label{fig:iso-perimeter-4}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=.66\textwidth]{pics_eps/0121_fourTriplesAllPlot}
    \caption{All 4- and 3-groups of Pythagorean triples with the same perimeter. They fall on common iso-perimeter level curves (red) in $(a,b)$ space.}
    \label{fig:iso-perimeter-3-and-4}
\end{figure}

==> appendices/102_app_orbit_vertices.tex <==
Let the boundary of the Billiard satisfy Equation~\eqref{eqn:billiard-f}. Assume, without loss of generality, that $a{\geq}b$.

Given a starting vertex $P_1$ and an exit angle $\alpha$ (as above), the orbit $P_1P_2P_3$ will be such that \cite{ronaldo19}:

vertex $P_2$ will be given by $(p_{2x},p_{2y})/q_2$, with

\begin{align*}
%\label{eqn:p2}
p_{2x}=&-{b}^{4} \left(  \left(   a^2+{b}^{2}\right)\cos^{2}\alpha   -{a}^{2}  \right) x_1^{3}-2\,{a}^{4}{b}^{2} \cos \alpha  \,\sin  \alpha  \,  x_1^{2}{y_1}\\
&+{a}^{4} \left(  ({a
}^{2}-3\, {b}^{2}) \cos^{2} \alpha  +{b}^{2}
 \right) {x_1}\,y_1^{2}-2{a}^{6} \,\cos  \alpha  \sin   \alpha  \, y_1^{3} ,
\\
p_{2y}=& 2{b}^{6} \,\cos \alpha\sin \alpha\,   x_1^{3}+{b}^{4}\left(  ({b
 }^{2}-3\, {a}^{2}) \cos^{2} \alpha  +{a}^{2}
  \right) x_1^{2}{y_1}\\
&+  2\,{a}^{2} {b}^{4}\cos \alpha \sin
  \alpha \; {x_1} y_1^{2} -{
a}^{4}  \left(  \left(   a^2+{b}^{2}\right)\cos^{2}  \alpha  -{b}^{2}  \right)  y_1^{3}
\\
q_2=&{b}^{4} \left( a^2-c^2\cos^2\alpha   \right)
x_1^{2}+{a}^{4} \left(  {b}^{2}+c^2\cos^2 \alpha  
 \right) y_1^{2}\\
 & - 2\, {a}^{2}{b}^{2}{c^2}\cos \alpha\sin \alpha \; {x_1}\,{
y_1}.
\end{align*}

and vertex $P_3$ will be given by $(p_{3x},p_{3y})/q_3$, with:

\begin{align*}
p_{3x}=& {b}^{4} \left( {a}^{2}- \left( {b}^{2}+{a}^{2} \right) \right)
 \cos^{2}  \alpha   x_1^{3} +2\,{a}^{4}{b}^{2} \cos  \alpha \sin \alpha\,   x_1^{2}{ y_1}\\
 &+{a}^{4} \left( 
  \cos^{2}  \alpha  \left( {a}^{2}-3\,{b}^{2}
 \right) +{b}^{2} \right) { x_1}\, y_1^{2} +2\, {a}^{6} 
 \cos \alpha\,\sin \alpha\, y_1^{3}
\\
p_{3y}=& -2\, {b}^{6} \cos \alpha\sin \alpha\, x_1^{3}+{b}^{4} \left( {a}^{2}+ \left( {b}^{2}-3\,{a}^{2} \right)    \cos^2\alpha \right) {{ x_1}}^{2}{ y_1}
\\
& -2\,{a}^{2}  {b}^{4}\cos
 \alpha  \sin \alpha\,  x_1 y_1^{2}+
 {a}^{4} \left( {b}^{2}- \left( {b}^{2}+{a}^{2} \right)   \cos^{2}  \alpha  \right)\,  y_1^{3},
\\
q_3=& {b}^{4} \left( {a}^{2}-{c^2}\cos^{2}\alpha   \right) x_1^{2}+{a}^{4} \left( {b}^{2}+c^2\cos^{2}\alpha  \right)  y_1^{2}\\
&+2\,{a}^{2}{b}^{
2} c^2 \cos\alpha \sin\alpha\, { x_1}\,{ y_1}.
\end{align*}

The sides of the triangular orbit have lengths 
$s_1=\mid P_3-P_2\mid$, $s_2=\mid P_3-P_1\mid$ and
$s_3=\mid P_2-P_1\mid$.
